Elliptic polylogarithms and Feynman parameter integrals

In this paper we study the calculation of multiloop Feynman integrals that cannot be expressed in terms of multiple polylogarithms. We show in detail how certain types of two- and three-point functions at two loops, which appear in the calculation of higher order corrections in QED, QCD and in the electroweak theory (EW), can naturally be expressed in terms of a recently introduced elliptic generalisation of multiple polylogarithms by direct integration over their Feynman parameter representation. Moreover, we show that in all examples that we considered a basis of pure Feynman integrals can be found.

==> kite_equal_masses.tex <==
% !TEX root = 3ptFunctions.tex

\section{Kite}
\label{sec:kite}
\LT{Here should come the Kite with different masses?}
Using the same formalism, we have also computed the kite integral shown in fig.~\ref{}
\beq\bsp
K&(p^2,m_1^2,m_2^2,m_3^2)\\
 &= -\frac{e^{2\gamma_E\eps}}{\pi^D}\, \int \frac{d^D k\, d^D l}{l^2\, (k-p)^2\, (k^2-m_1^2) ((k-l)^2-m_2^2) ((l-p)^2-m_3^2)}\,,
\label{eq:kite}
\esp\eeq

\begin{equation}
K(p^2,m^2) \equiv K(p^2,m^2,m^2,m^2) \,.
\end{equation}


\begin{equation}
\vec{a} = \left\{ \frac{1}{2} \left( 1 - \sqrt{1+\rho}\right),  \frac{1}{2} \left( 1 + \sqrt{1+\rho}\right),
\frac{1}{2} \left( 1 - \sqrt{1+\bar{\rho}}\right),  \frac{1}{2} \left( 1 + \sqrt{1+\bar{\rho}}\right)\right\}\,.
\end{equation}
\beq
K(p^2,m^2) = \frac{1}{m^4} 
\frac{1}{z}\left[ K_0(z) + \mathcal{O}(\epsilon) \right]
\eeq

\begin{align}
K_0(z) &= 
\frac{1}{6} \Big[-9 \cEf{-1 & -1 & 1}{0 & 0 & 1 }{1}
-9 \cEf{-1 & -1 & 1 }{0 & 1 & 1 }{1}
-18 \cEf{-1 & -1 & 1 }{0 & \infty  & 1 }{1}
-9 \cEf{-1 & 1 & -1 }{0 & 1 & 0 }{1} \nonumber \\&
-9 \cEf{-1 & 1 & -1 }{0 & 1 & 1 }{1}
-18 \cEf{-1 & 1 & -1 }{0 & 1 & \infty  }{1}
+3 \cEf{-1 & -1 & 1 }{\infty  & 0 & 1 }{1}
+3 \cEf{ -1 & -1 & 1 }{\infty  & 1 & 1 }{1} \nonumber \\&
+6 \cEf{-1 & -1 & 1 }{\infty  & \infty  & 1 }{1}
+3 \cEf{-1 & 1 & -1 }{\infty  & 1 & 0 }{1}
+3 \cEf{-1 & 1 & -1 }{\infty  & 1 & 1 }{1}
+6 \cEf{-1 & 1 & -1 }{\infty  & 1 & \infty  }{1} \nonumber \\&
+3 \cEf{1 & -1 & -1 }{0 & 0 & 0 }{1}
+3 \cEf{1 & -1 & -1 }{0 & 0 & 1 }{1}
+6 \cEf{1 & -1 & -1 }{0 & 0 & \infty  }{1}
-6 \cEf{1 & -1 & -1 }{0 & 1 & 0 }{1} \nonumber \\&
-6 \cEf{1 & -1 & -1 }{0 & 1 & 1 }{1}
-12 \cEf{1 & -1 & -1 }{0 & 1 & \infty  }{1}
-3 \cEf{1 & -1 & -1 }{0 & \infty  & 0 }{1}
-3 \cEf{1 & -1 & -1 }{0 & \infty  & 1 }{1} \nonumber \\&
-6 \cEf{1 & -1 & -1 }{0 & \infty  & \infty  }{1}
%-3 \cEf{1 & 1 & 1 }{0 & 0 & 0 }{1}
%+9 \cEf{1 & 1 & 1 }{0 & 0 & 1 }{1}
%+9 \cEf{1 & 1 & 1 }{0 & 1 & 0 }{1} \nonumber \\&
-6 \cEf{1 & -1 & -1 }{\xi & 0 & 0 }{1}
-6 \cEf{1 & -1 & -1 }{ \xi & 0 & 1 }{1}
-12 \cEf{1 & -1 & -1 }{ \xi & 0 & \infty  }{1} \nonumber \\&
+3 \cEf{ 1 & -1 & -1 }{ \xi & 1 & 0 }{1} 
+3 \cEf{1 & -1 & -1 }{\xi & 1 & 1 }{1}
+6 \cEf{1 & -1 & -1 }{\xi & 1 & \infty  }{1} \nonumber \\&
+9 \cEf{1 & -1 & -1 }{\xi & \infty  & 0 }{1}
+9 \cEf{1 & -1 & -1 }{ \xi & \infty  & 1 }{1} 
+18 \cEf{1 & -1 & -1 }{ \xi & \infty  & \infty  }{1}\nonumber \\& 
+6 \cEf{1 & 1 & 1 }{\xi & 0 & 0 }{1} 
-2 \pi ^2 G(0;z)+ \pi ^2 G(1;z) 
-3 G(0,0,0;z)+6 G(0,1,0;z) \nonumber \\& -12 G(0,1,1;z)+3 G(1,0,0;z) +6 G(1,0,1;z)+27 \zeta_3\Big]\nonumber \\&
%%%%%%%
+ 2\pi i \Big[2 
\cEf{1 & 0 & -1}{ \xi & 0 & \infty  }{1}
 +\cEf{1 & 0 & -1}{\xi & 0 & 0 }{1}
 +\cEf{1 & 0 & -1}{ \xi & 0 & 1 }{1}
 +2 \cEf{0 & -1 & 1}{ 0 & \infty  & 1 }{1} \nonumber \\& \qquad  \;\;\,
 +2 \cEf{0 & 1 & -1}{ 0 & 1 & \infty  }{1}
 +\cEf{0 & -1 & 1}{ 0 & 0 & 1 }{1}
 +\cEf{0 & -1 & 1}{ 0 & 1 & 1 }{1}
 +\cEf{0 & 1 & -1}{ 0 & 1 & 0 }{1}\nonumber \\&  \qquad  \;\;\,
 +\cEf{0 & 1 & -1}{ 0 & 1 & 1 }{1} \Big]\,, \label{eq:kitecE4}
\end{align}
where we defined $\xi = 1/(1-z)$.

==> motivation.tex <==
% !TEX root = 3ptFunctions.tex

\section{Feynman integrals beyond multiple polylogarithms}
\label{sec:motivation}

An important part of the success of the high energy physics community in handling increasingly
complicated multiloop calculations is undoubtedly due to our deep understanding of the properties of multiple polylogarithms.
Typically, complicated Feynman integrals are computed by means of two apparently orthogonal methods.
On the one hand, one can attempt their direct integration over some integral representation (for example in terms
of Feynman parameters or Mellin-Barnes integrals). On the other, one can derive differential equations satisfied by the Feynman
integrals and try to solve them.
Understanding the properties of MPLs has been a crucial step to systematise both strategies.
For what concerns direct integration techniques, the highest point of this program   has been reached with the 
enunciation of the criterion of linear reducibility~\cite{Brown:2008um,Panzer:2015ida}. This method allows one to define a 
(quite general) class of Feynman integrals which can be algorithmically expressed in terms of MPLs
by direct integration over their Feynman-parameter representation.
A similarly important result in the context of the differential-equation method 
(even if mathematically less rigorous) is the concept of 
canonical basis of master integrals~\cite{Henn:2013pwa}. Canonical master integrals
fulfil differential equations which admit solutions in terms of iterated integrals 
over particularly simple kernels, which can be expressed as total differentials of logarithms.
If there exists a parametrisation of the external kinematics in terms of which the 
arguments of the logarithms are all rational functions,
the corresponding iterated integrals can be straightforwardly expressed in terms of MPLs. 
Indeed, both by direct integration through the linear reducibility criterion, and in the case of canonical differential 
equations\footnote{In the absence of square roots which cannot be rationalised.},  
one ends up with iterated integrals in a set of variables,
say $x$ for simplicity, over rational functions $R(x)$. It is then 
a well-known fact that the space defined by these integrals 
is spanned by linear combinations of MPLs and rational functions.

Generalising these ideas beyond MPLs has been a very pressing issue, both for their potential phenomenological impact,
in particular in collider physics,
and also for their conceptual relevance.
In the last years significant steps have been taken in extending both strategies (i.e. direct integration and differential equations)
to the so-called elliptic case, namely when the natural geometry associated to the Feynman graphs under consideration has genus equal to one.
The scope of this paper is to show how, by using the class of functions defined in refs.~\cite{Broedel:2018qkq,Broedel:2017siw,Broedel:2017kkb}, 
the algorithms for the direct integration of Feynman integrals can be suitably generalised to the elliptic case.
We developed a machinery which allows us to treat those classes of Feynman integrals which do not 
fulfil the criterion of linear reducibility and, instead,
require dealing with iterated integrals over more general
rational functions $R(x,y)$, where $y=\sqrt{P(x)}$ defines an elliptic curve\footnote{In this case, $P(x)$ can be an irreducible cubic or quartic polynomial.}.
We stress here that, in order for our approach to be successful, one must deal with integrals where one and only elliptic curve
appears and no other square roots are present. 
It is possible to draw a parallel between our approach and the idea of ``elliptic linear reducibility'' recently put forward in~\cite{Hidding:2017jkk}.
There, a generalisation of the criterion of linear reducibility to the elliptic case is attempted.
\todo{Rephrase} Our approach is different in at least two aspects. First, since we believe that the investigation of these integrals is still in its 
infancy, we do not aim to provide general criteria which would generalise the (rigorous) criterion of linear reducibility to the elliptic case.
Second, and more importantly, we work with a well defined class of functions whose algebraic properties can be studied
rigorously and whose transcendental weight can be defined. This provides us also with the unique opportunity 
to confirm the conjectures about the existence of
pure bases of Feynman integrals, beyond the polylogarithmic world. Indeed, we will verify explicitly that for all the examples considered,
a pure basis of functions can always be found.

Before diving into the computations, one more comment is in order.
It is very clear to us that, even at two loops, the class of functions that we are considering will probably not be the end of the story, since either 
multiple elliptic curves can appear~\cite{Adams:2018bsn,Adams:2018kez},
or entirely new geometrical objects~\cite{Bloch:2014qca,Primo:2017ipr,Bourjaily:2017bsb,Bourjaily:2018ycu,Bourjaily:2018yfy}. 
Still, with this paper we aim to show that our
framework is general and flexible enough to cover many problems of direct physical interest and, therefore, deserves
to be developed further.
We will show explicitly how different  two- and three-point functions at two loops can be integrated in terms of eMPLs,
discussing thoroughly the details of the manipulations required to bring the integrals to the correct form.
We postpone to future publications the extend these techniques to the study of some two-loop four-point Feynman integrals.







%
%It is well known that given an iterated integral, if at every integration step the integrand can be brought to 
%a form where it is a rational function with at most simple poles in the integration variable, the result of this 
%integral is a combination of MPLs. In order for this to be achieved, techniques like partial fractioning and rational 
%changes of variables may need to be employed in order to bring the integrand to the form \eqref{eq:Mult_PolyLog_def}. 
%
%There are situations, however, where square roots of irreducible polynomials of degree higher than two appear 
%in the integrand at a given step. When this occurs and no change of variables is found that rationalises the square root, 
%this falls out of the scope of MPLs and one must find alternatives. Up to very recently, apart from very special 
%cases, at this point the only hope was to compute the integral as a series expansion around certain 
%parameters or via differential equations, and a general-purpose set of function that is natural to express these integrals was lacking.
%
%In between MPLs and the completely generic case, one may consider integrals which have a 
%dependence on a single square root of a polynomial of degree $n=3,4$, i.e. an elliptic curve. 
%In this situation, the eMPLs reviewed in the previous section are the generalisation of MPLs that 
%allow any integral of this kind to be computed using the very same techniques known from the polylogarithmic case. 
%At each step in the integration, one simply needs to partial fraction the integrand and fit it into a 
%combination of the integration kernels $\Psi_n$ entering the definition \eqref{eq:cE4_def}. 
%Although technically more involved that the MPL case, conceptually it is just as general and powerful.
%\todo[inline]{Paragraph with relation to other work, Moriello etc}
%
%We show explicitly in the following sections several applications of this method, 
%demonstrating that this one class of functions is sufficient to give analytical results for 
%several distinct integrals. This is of course not the end of the story, as there are situations 
%where multiple elliptic curves appear \cite{Adams:2018bsn,Adams:2018kez} and integrals 
%which involve square roots of polynomials of higher degree~\cite{Bourjaily:2017bsb,Bourjaily:2018ycu,Bourjaily:2018yfy}. 
%eMPLs however, are sufficient to tackle a wide range of functions which are relevant for applications in particle physics.
